Self-supervised Pretraining and Transfer Learning Enable Flu and COVID-19 Predictions in Small Mobile Sensing Datasets

Detailed mobile sensing data from phones, watches, and fitness trackers offer an unparalleled opportunity to quantify and act upon previously unmeasurable behavioral changes in order to improve individual health and accelerate responses to emerging diseases. Unlike in natural language processing and computer vision, deep representation learning has yet to broadly impact this domain, in which the vast majority of research and clinical applications still rely on manually defined features and boosted tree models or even forgo predictive modeling altogether due to insufficient accuracy. This is due to unique challenges in the behavioral health domain, including very small datasets (~10^1 participants), which frequently contain missing data, consist of long time series with critical long-range dependencies (length>10^4), and extreme class imbalances (>10^3:1). Here, we introduce a neural architecture for multivariate time series classification designed to address these unique domain challenges. Our proposed behavioral representation learning approach combines novel tasks for self-supervised pretraining and transfer learning to address data scarcity, and captures long-range dependencies across long-history time series through transformer self-attention following convolutional neural network-based dimensionality reduction. We propose an evaluation framework aimed at reflecting expected real-world performance in plausible deployment scenarios. Concretely, we demonstrate (1) performance improvements over baselines of up to 0.15 ROC AUC across five prediction tasks, (2) transfer learning-induced performance improvements of 16% PR AUC in small data scenarios, and (3) the potential of transfer learning in novel disease scenarios through an exploratory case study of zero-shot COVID-19 prediction in an independent data set. Finally, we discuss potential implications for medical surveillance testing.

==> 0b-introduction_old.tex <==
old abstract

While neural representation learning, and in particular large pretrained models, have revolutionized research and applications in natural language processing and computer vision, this has not yet been the case for behavioral health modeling (e.g., the prediction of health outcomes from wearable time series data). 
This is in part because the domain's datasets are significantly smaller and commonly exhibit a large context sizes, a large degree of missingness and extreme class imbalances.
%
Therefore, off-the-shelf deep learning models require significant, often prohibitive, adaptation. Accordingly, the vast majority of research and clinical applications still rely on manually defined features with boosted tree models, or refrain from learning predictive models altogether as current solutions cannot provide satisfactory performance given the limited training data. % and other challenges.

Here, we address these challenges by providing a neural architecture framework designed for behavioral health data that can learn generalizable feature representations from raw time series and demonstrates the feasibility of transfer learning on small data domains through fine tuning.
This architecture combines benefits from Convolutional and Transformer architectures to \mike{rewrite to match results} enable better prediction performance by learning directly from raw minute-level sensor data without the need for handcrafted features by up to 0.15 ROC AUC \tim{revisit what to cite here}, and (2) use pretraining to outperform simpler neural models and boosted decision trees by predicting COVID-19 diagnosis with XX ROC AUC in an independently collected dataset.


\section{Introduction}

In recent years, deep learning has provided significant performance improvements across NLP and computer vision \citationneeded. However, most off-the-shelf methods require large datasets, which has slowed their adoption in behavioral modeling applications such as mobile sensing or behavioral health \tim{need to decide on buzzwords} where researchers report difficulties collecting labeled datasets of even dozens of participants \cite{xu2021understanding}. Without substantial funding for personnel and devices data collection quickly scales to an arduous process of recruiting and paying participants, debugging devices, and monitoring data quality. Therefore, researchers have historically often been limited to using small datasets, hand-crafted features, and less data hungry and more easily adaptable non-neural models~\cite{xu2021understanding,laport-lopez_review_2020}. \tim{ideally add 5+++ more citations here}
\tim{need to say more about why this task is important -- why do we care about small mobile sensing studies etc? motivate from health angle, perhaps say that there are no large studies}
\tim{need to connect this space to multimodal time series classification on long time series (e.g. min by min steps,hr,sleep data}

If mobile sensing applications could achieve improved performance and generalizability with smaller datasets they could be deployed quickly in situations with limited training data. For example, in the crucial early days of a emerging disease outbreak, such as the COVID-19 pandemic, laboratory testing may not be widely available, and many positive cases may remain undetected. In this setting, a highly generalizable model could be trained on what few positive test results a researcher had, and used to identify members of a population who may be infected and should be targeted for additional testing. \citationneeded %maybe one of the covid +fitbit papers?

In this paper we enable these conditions \tim{make more precise?} through transfer learning, which has recently driven advancements in NLP and  computer vision \cite{devlin2019bert,lan2019albert,mikolov2013distributed,krizhevsky2012alexnet,he2016resnet}. In each case, a researcher first obtains a model trained on a large, more readily available, task-independent dataset (such as the popular language model BERT, which was trained in part on Wikipedia) and finetunes it on a typically smaller task-specific dataset. The resulting finetuned model provides higher predictive power than either the pretrained model without finetuning or a model trained exclusively on the smaller dataset. However, existing architectures and pretraining techniques cannot trivially accept high dimensional, heterogeneous multi-modal timeseries data, and are not equipped to support missing data, both of which are rare in computer vision and NLP but endemic in behavioral modeling applications  \cite{xu2021understanding}.
\mike{Work in the "framework" motivation here}

\mike{Want some way of saying "new to the field" in here, but not sure how to squeeze it in}
To this end, we first describe a multi-modal timeseries classification model which learns directly from raw minute-level sensor data, combines the hierarchical feature extraction of CNNs with the scalability \tim{ability to learn long-range dependencies} of transformers, and incorporates information about missing data (Section~\ref{subsec:model}). Next, we describe three novel \tim{need to back this up directly in related work -- say what tasks others did. question could come up why we did not compare to those though.} self-supervised pretraining tasks for behavioral data, which enable large-scale pretraining without the need for exogenous labels (Section~\ref{subsec:self_supervised_tasks}). 

We present a new framework for evaluating behavioral models, which provides guidelines for selecting substantive tasks and evaluation metrics, and reduces the statistical uncertainty introduced by inherent extreme class imbalances (Section~\ref{sec:evaluation}). Then, we evaluate our model on five highly realistic single domain prediction tasks related to predicting the flu with FitBit data, and show that CNN encoders, transformer blocks, modeling missingness, and self-supervised pretraining significantly increase predictive power (Section~\ref{subsec:pred_tasks}). Next, we compare three self-supervised pretraining tasks and show that a tasks which incorporates domain-inspired expertise performs best (Section \ref{subsec:results_pretraining}). 

\tim{make own paragraph}
We also successfully show that transfer learning permits models to learn in new domains with limited data by finetuning a model to predict COVID-19 diagnosis with 0.62 ROC AUC with data from only ten users (Section ~\ref{subsec:domain_transfer}). Then, we show that our model supports the reuse of large, unlabeled datasets by simulating a common setting where researchers have access to small pools of labeled data.

Finally, we situate our model in the context of medical literature on surveillance testing to show that our model provides predictions on-par with rapid antigen testing \tim{too much? comparable to some COVID-19 rapid antigen testing approaches?} (Section ~\ref{sec:discussion}).

\tim{make model publicly available at anonymized...}
\tim{should discuss w luca about pretrained model public}

==> 2-datasets.tex <==
\section{Datasets}
